Simplicity by Obfuscation: Evaluating LLM-Driven Code Transformation with Semantic Elasticity

Code obfuscation is the conversion of original source code into a functionally equivalent but less readable form, aiming to prevent reverse engineering and intellectual property theft. This is a challenging task since it is crucial to maintain functional correctness of the code while substantially disguising the input code. The recent development of large language models (LLMs) paves the way for practical applications in different domains, including software engineering. This work performs an empirical study on the ability of LLMs to obfuscate Python source code and introduces a metric (i.e., semantic elasticity) to measure the quality degree of obfuscated code. We experimented with 3 leading LLMs, i.e., Claude-3.5-Sonnet, Gemini-1.5, GPT-4-Turbo across 30 Python functions from diverse computational domains. Our findings reveal GPT-4-Turbo's remarkable effectiveness with few-shot prompting (81% pass rate versus 29% standard prompting), significantly outperforming both Gemini-1.5 (39%) and Claude-3.5-Sonnet (30%). Notably, we discovered a counter-intuitive "obfuscation by simplification" phenomenon where models consistently reduce rather than increase cyclomatic complexity. This study provides a methodological framework for evaluating AI-driven obfuscation while highlighting promising directions for leveraging LLMs in software security.

==> src/threats.tex <==

Internal validity threats concern our experimental setup. While we included 30 diverse functions from established repositories, they may not represent all programming patterns. Even though the selected models represent current state-of-the-art, we left out open-source LLM from our analysis since we focus on proprietary ones for security issues. Nevertheless, our methodology can be applied to every LLM architecture as we didn't use any peculiar feature of the considered LLMs. Our metrics, while comprehensive, cannot capture all aspects of obfuscation quality. The proposed Semantic Elasticity metric has not been validated across different contexts and coding paradigms and should be considered an initial exploration rather than a definitive measurement.

External validity relates to generalizability. Our focus on Python code may limit applicability to other languages with different paradigms or syntax structures \cite{balakrishnan2018}. Real-world applications often involve complex interactions between multiple components, while our evaluation focused on isolated functions \cite{herraiz2011beyond}. We evaluated obfuscation effectiveness primarily through code structure metrics rather than resistance to actual deobfuscation attempts, which could provide a more complete assessment of protection effectiveness.
